SEAT: Stable and Explainable Attention

Currently, attention mechanism becomes a standard fixture in most state-of-the-art natural language processing (NLP) models, not only due to outstanding performance it could gain, but also due to plausible innate explanation for the behaviors of neural architectures it provides, which is notoriously difficult to analyze. However, recent studies show that attention is unstable against randomness and perturbations during training or testing, such as random seeds and slight perturbation of embedding vectors, which impedes it from becoming a faithful explanation tool. Thus, a natural question is whether we can find some substitute of the current attention which is more stable and could keep the most important characteristics on explanation and prediction of attention. In this paper, to resolve the problem, we provide a first rigorous definition of such alternate namely SEAT (Stable and Explainable Attention). Specifically, a SEAT should has the following three properties: (1) Its prediction distribution is enforced to be close to the distribution based on the vanilla attention; (2) Its top-k indices have large overlaps with those of the vanilla attention; (3) It is robust w.r.t perturbations, i.e., any slight perturbation on SEAT will not change the prediction distribution too much, which implicitly indicates that it is stable to randomness and perturbations. Finally, through intensive experiments on various datasets, we compare our SEAT with other baseline methods using RNN, BiLSTM and BERT architectures via six different evaluation metrics for model interpretation, stability and accuracy. Results show that SEAT is more stable against different perturbations and randomness while also keeps the explainability of attention, which indicates it is a more faithful explanation. Moreover, compared with vanilla attention, there is almost no utility (accuracy) degradation for SEAT.

==> SEAT_ Stable and Explainable Attention/figures/examples/embedding.tex <==

% code of example
\tikzset{
    %Define standard arrow tip
    >=stealth',
    %Define style for boxes
    punkt/.style={
          very thick,
          rectangle split,
          rectangle split parts=2,
          inner ysep=1.2mm,
          inner xsep=1.5mm,
          rounded corners,
          draw=black, thick,
          text width=9.3cm},
    punx/.style={
          rectangle,
          rounded corners,
          align=left,
          text width=0.55cm,
          text depth=0.01cm,
          draw=white},
  header/.style = {%
    inner ysep = +1.5em,
    append after command = {
      \pgfextra{\let\TikZlastnode\tikzlastnode}
      node [header node] (header-\TikZlastnode) at (\TikZlastnode.north) {#1}
      node [span = (\TikZlastnode)(header-\TikZlastnode)]
        at (fit bounding box) (h-\TikZlastnode) {}
    }
  },
}
\begin{tikzpicture}[scale=1.0]
\node[punkt](Vanilla){
\Textbox{0.1cm}{\textbf{Vanilla} \quad \textbf{JSD.$\downarrow$} = 0.024 \quad \textbf{TVD.$\downarrow$} = 2.321}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})
}\\
{\centering \small \textbf{Perturbed}: 
\colorword{pink!100}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!20}{black}{horrible}
($99.9\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Vanilla](Word-AT){
\Textbox{0.1cm}{\textbf{Word-AT} \quad \textbf{JSD.} = 0.078 \quad \textbf{TVD.} = 0.04}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% \colorword{pink}{black}{This} film is just plain {horrible}.
\colorword{pink!100}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!20}{black}{horrible}
($97.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\node[punkt, below=0cm of Word-AT](Att-AT){
\Textbox{0.1cm}{\textbf{Att-AT} \quad \textbf{JSD.} = 0.016 \quad \textbf{TVD.} = 0.237}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% {This} film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!60}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!70}{black}{horrible}
($67.9\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Att-AT](Ours){
\Textbox{0.1cm}{\textbf{Ours} \quad \textbf{JSD.} = 4.3e-7 \quad \textbf{TVD.} = 0.001}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!23}{black}{This} \colorword{pink!18}{black}{film} 
\colorword{pink!13}{black}{is} 
\colorword{pink!28}{black}{just}
\colorword{pink!48}{black}{plain} \colorword{pink!98}{black}{horrible}
($97.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\end{tikzpicture}

==> SEAT_ Stable and Explainable Attention/figures/examples/seed.tex <==

% code of example
\tikzset{
    %Define standard arrow tip
    >=stealth',
    %Define style for boxes
    punkt/.style={
          very thick,
          rectangle split,
          rectangle split parts=2,
          inner ysep=1.2mm,
          inner xsep=1.5mm,
          rounded corners,
          draw=black, thick,
          text width=9.3cm},
    punx/.style={
          rectangle,
          rounded corners,
          align=left,
          text width=0.55cm,
          text depth=0.01cm,
          draw=white},
  header/.style = {%
    inner ysep = +1.5em,
    append after command = {
      \pgfextra{\let\TikZlastnode\tikzlastnode}
      node [header node] (header-\TikZlastnode) at (\TikZlastnode.north) {#1}
      node [span = (\TikZlastnode)(header-\TikZlastnode)]
        at (fit bounding box) (h-\TikZlastnode) {}
    }
  },
}
\begin{tikzpicture}[scale=1.0]
\node[punkt](Vanilla){
\Textbox{0.1cm}{\textbf{Vanilla} \quad \textbf{JSD.$\downarrow$} = 0.008 \quad \textbf{TVD.$\downarrow$} = 0.172}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})
}\\
{\centering \small \textbf{Perturbed}: 
\colorword{pink!20}{black}{This} \colorword{pink!30}{black}{film} 
\colorword{pink!40}{black}{is} 
\colorword{pink!54}{black}{just}
\colorword{pink!20}{black}{plain} \colorword{pink!40}{black}{horrible}
($97.9\%\rightarrow$\textcolor{red}{\textcolor{blue}{Neg.}})}
};
\node[punkt, below=0cm of Vanilla](Word-AT){
\Textbox{0.1cm}{\textbf{Word-AT} \quad \textbf{JSD.} = 0.013 \quad \textbf{TVD.} = 0.080}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% \colorword{pink}{black}{This} film is just plain {horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!30}{black}{film} 
\colorword{pink!40}{black}{is} 
\colorword{pink!54}{black}{just}
\colorword{pink!20}{black}{plain} \colorword{pink!40}{black}{horrible}
($98.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\node[punkt, below=0cm of Word-AT](Att-AT){
\Textbox{0.1cm}{\textbf{Att-AT} \quad \textbf{JSD.} = 0.005 \quad \textbf{TVD.} = 0.189}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% {This} film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!40}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!50}{black}{horrible}
($95.9\%\rightarrow$\textcolor{red}{\textcolor{blue}{Neg.}})}
};
\node[punkt, below=0cm of Att-AT](Ours){
\Textbox{0.1cm}{\textbf{Ours} \quad \textbf{JSD.} = 6.5e-6 \quad \textbf{TVD.} = 0.013}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!30}{black}{This} \colorword{pink!25}{black}{film} 
\colorword{pink!13}{black}{is} 
\colorword{pink!28}{black}{just}
\colorword{pink!48}{black}{plain} \colorword{pink!98}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\end{tikzpicture}

==> SEAT_ Stable and Explainable Attention/figures/examples/setup.tex <==

\colorlet{red1}{red}
\colorlet{red2}{red!50}
\colorlet{red3}{red!25}
\colorlet{blue1}{blue}
\colorlet{blue2}{blue!50}
\colorlet{blue3}{blue!25}
\makeatletter
\pgfdeclaregenericanchor{top base}{%
  \csname pgf@anchor@#1@north\endcsname
  \pgf@anchor@generic@top@base@main
}
\pgfdeclaregenericanchor{top base west}{%
  \csname pgf@anchor@#1@north west\endcsname
  \pgf@anchor@generic@top@base@main
}
\pgfdeclaregenericanchor{top base east}{%
  \csname pgf@anchor@#1@north east\endcsname
  \pgf@anchor@generic@top@base@main
}
\def\pgf@anchor@generic@top@base@main{%
  {%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y-\pgf@ya
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y-\pgf@ya
    \pgf@ya=0pt
    \pgfutil@loop
    \ifdim\pgf@y>\baselineskip
      \advance\pgf@y-\baselineskip
      \advance\pgf@ya\baselineskip
    \pgfutil@repeat
    \global\pgf@y=\pgf@ya
  }%
}
\makeatother
\newcommand\Textbox[2]{%
    \parbox[c][#1][c]{6.7cm}{#2}}


==> SEAT_ Stable and Explainable Attention/figures/examples/word.tex <==

% code of example
\tikzset{
    %Define standard arrow tip
    >=stealth',
    %Define style for boxes
    punkt/.style={
          very thick,
          rectangle split,
          rectangle split parts=2,
          inner ysep=1.2mm,
          inner xsep=1.5mm,
          rounded corners,
          draw=black, thick,
          text width=9.3cm},
    punx/.style={
          rectangle,
          rounded corners,
          align=left,
          text width=0.55cm,
          text depth=0.01cm,
          draw=white},
  header/.style = {%
    inner ysep = +1.5em,
    append after command = {
      \pgfextra{\let\TikZlastnode\tikzlastnode}
      node [header node] (header-\TikZlastnode) at (\TikZlastnode.north) {#1}
      node [span = (\TikZlastnode)(header-\TikZlastnode)]
        at (fit bounding box) (h-\TikZlastnode) {}
    }
  },
}
\begin{tikzpicture}[scale=1.0]
\node[punkt](Vanilla){
\Textbox{0.1cm}{\textbf{Vanilla} \quad \textbf{JSD.$\downarrow$} = 0.012 \quad \textbf{TVD.$\downarrow$} = 0.230}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})
}\\
{\centering \small \textbf{Perturbed}: 
\colorword{pink!30}{black}{This} \colorword{pink!20}{black}{\textbf{movie}} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!50}{black}{\textbf{terrible}}($59.2\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Vanilla](Word-AT){
\Textbox{0.1cm}{\textbf{Word-AT} \quad \textbf{JSD.} = 0.014 \quad \textbf{TVD.} = 0.080}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% \colorword{pink}{black}{This} film is just plain {horrible}.
\colorword{pink!30}{black}{This} \colorword{pink!30}{black}{\textbf{movie}} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!50}{black}{\textbf{terrible}}($99.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\node[punkt, below=0cm of Word-AT](Att-AT){
\Textbox{0.1cm}{\textbf{Att-AT} \quad \textbf{JSD.} = 0.004 \quad \textbf{TVD.} = 0.260}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!10}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!80}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% {This} film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{\textbf{movie}} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!30}{black}{plain} \colorword{pink!60}{black}{\textbf{terrible}}($56.8\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Att-AT](Ours){
\Textbox{0.1cm}{\textbf{Ours} \quad \textbf{JSD.} = 8.4e-8 \quad \textbf{TVD.} = 0.012}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!23}{black}{This} \colorword{pink!18}{black}{\textbf{movie}} 
\colorword{pink!13}{black}{is} 
\colorword{pink!28}{black}{just}
\colorword{pink!48}{black}{plain} \colorword{pink!96}{black}{\textbf{terrible}}($98.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\end{tikzpicture}

==> SEAT_ Stable and Explainable Attention/figures/overview.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{figures/overview.pdf}
\caption{An illustration of an attention heatmap for a BiLSTM model with attention mechanisms and the model with REAL-attention. The proposed REAL-attention is more explainable for attention score and more stable for output distribution.}
\label{fig:overview}
\end{figure}

==> SEAT_ Stable and Explainable Attention/figures/seeds_main.tex <==
\begin{figure*}[ht]
    \centering
    \small
    \begin{tabular}{cccc}
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/baseline/emotion-simple-rnn+tanh-seed-diffs.pdf}
        & 
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/baseline/sst-simple-rnn+tanh-seed-diffs.pdf} &
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/baseline/hate-simple-rnn+tanh-seed-diffs.pdf}
        & 
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/baseline/rotten_tomatoes-simple-rnn+tanh-seed-diffs.pdf} \\
        (a) Baseline-\textsc{Emotion} & (b) Baseline-SST  &
        (c) Baseline-Hate & (d) Baseline-RottenT \\
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/ours/Emotion-simple-rnn+ours-seed-diffs.pdf}
        & 
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/ours/sst-simple-rnn+ours-seed-diffs.pdf} &
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/ours/hate-simple-rnn+ours-seed-diffs.pdf}
        & 
        \includegraphics[width=3.5cm,height=0.12\textheight]{figures/seed/ours/rotten_tomatoes-simple-rnn+ours-seed-diffs.pdf} \\
        (e) Ours-\textsc{Emotion} & (f) Ours-SST  &
        (g) Ours-Hate & (h) Ours-RottenT \\
    \end{tabular}
    \caption{Comparison of stability against random seeds for vanilla attention and SEAT. Densities of maximum JS divergences (x-axis) as a function of the max attention (y-axis) in each instance
between its base model and models initialized on different random seeds. In each max-attention
bin, top (blue) is a negative-label instance, and bottom (red) is a positive-label instance.
%Comparison of densities of maximum JSD (x-axis) as a function of the max attention (y-axis) in each instance between the base distributions and: (a-d) baseline models (vanilla) initialized on different random seeds in Emotion, SST, Hate and RottenT datasets respectively; (e-h) are our SEAT initialized on different random seeds in corresponding datasets. In each max-attention bin, top (blue) is the negative-label instances, bottom (red) is positive-label instances. All results are conducted with RNN architecture.
\label{fig:seeds_main}}
\end{figure*}

==> SEAT_ Stable and Explainable Attention/tab/ablation.tex <==
\begin{table}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccc} 
\toprule
\multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Ablation Setting}} & \multicolumn{3}{c}{\textbf{Metrics}}                       \\ 
\cmidrule(l){2-6}
                        & \bm{$\mathcal{L}_3$}     & \bm{$\mathcal{L}_{Topk}$}            & \textbf{JSD$\downarrow$} & \textbf{TVD$\downarrow$} & \textbf{F1$\uparrow$}  \\ 
\midrule
\multirow{4}{*}{\textbf{RNN}}    &           &                          & 0.025           & 21.464          & \textbf{0.814}         \\
                        & $\rightt$ &                          & 0.017           & 1.966           & 0.804         \\
                        &           & $\rightt$                & 8.21E-08        & 2.997           & 0.782         \\
                        & $\rightt$ & $\rightt$                & \textbf{6.98E-08}        & \textbf{1.275}           & 0.813         \\ 
\midrule
\multirow{4}{*}{\textbf{BiLSTM}} &           &                          & 0.059           & 20.398          & \textbf{0.809}         \\
                        & $\rightt$ &                          & 0.033           & 1.214           & 0.802         \\
                        &           & $\rightt$                & 0.030           & 1.745           & 0.779         \\
                        & $\rightt$ & $\rightt$                & \textbf{0.028}           & \textbf{1.095}           & 0.801         \\ 
\midrule
\multirow{4}{*}{\textbf{BERT}}   &           &                          & 0.140           & 2.617           & \textbf{0.912}         \\
                        & $\rightt$ &                          & 0.114           & 0.056           & 0.909         \\
                        &           & $\rightt$                & 0.006           & 0.157           & 0.907         \\
                        & $\rightt$ & $\rightt$                & \textbf{2.49E-07}        & \textbf{0.028}           & 0.909         \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of the proposed method. We evaluate the effectiveness of the third term $\mathcal{L}_3$ and the second term $\mathcal{L}_{Topk}$ in (\ref{eq:6}) on three different architectures. JSD, TVD and F1 are reported to measure the stability and performance of the model. Here we conduct perturbation on the embedding space with radius of 0.01 on SST dataset.}
\label{tab:ablation}
\end{table}




==> SEAT_ Stable and Explainable Attention/tab/ablation_main.tex <==
\begin{table}[thbp]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccccc} 
\toprule
\multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Ablation Setting}} & \multicolumn{3}{c}{\textbf{Metrics}}                       \\ 
\cmidrule(l){2-6}
                        & \bm{$\mathcal{L}_3$}     & \bm{$\mathcal{L}_{Topk}$}            & \textbf{Suff.$\downarrow$} & \textbf{TVD$\downarrow$} & \textbf{F1$\uparrow$}  \\ 
\midrule
\multirow{4}{*}{\textbf{RNN}}    &           &                          & 7.02E-04           & 21.464          & \textbf{0.814}         \\
                        & $\rightt$ &                          & 6.22E-04           & 1.966           & 0.804         \\
                        &           & $\rightt$                & 2.22E-04        & 2.997           & 0.782         \\
                        & $\rightt$ & $\rightt$                & \textbf{1.02E-04}        & \textbf{1.275}           & 0.813         \\ 
\midrule
\multirow{4}{*}{\textbf{BiLSTM}} &           &                          & 0.255           & 20.398          & \textbf{0.809}         \\
                        & $\rightt$ &                          & 0.016           & 1.214           & 0.802         \\
                        &           & $\rightt$                & 0.004           & 1.745           & 0.779         \\
                        & $\rightt$ & $\rightt$                & \textbf{4.37E-06}           & \textbf{1.095}           & 0.801         \\ 
\midrule
\multirow{4}{*}{\textbf{BERT}}   &           &                          & 0.310           & 2.617           & \textbf{0.912}         \\
                        & $\rightt$ &                          & 0.280           & 0.056           & 0.909         \\
                        &           & $\rightt$                & 0.090           & 0.157           & 0.907         \\
                        & $\rightt$ & $\rightt$                & \textbf{0.019}        & \textbf{0.028}           & 0.909         \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of SEAT. We evaluate the effectiveness of $\mathcal{L}_3$ and  $\mathcal{L}_{Topk}$ in (\ref{eq:6}). %Suff. represents the interpretability of models. TVD and F1 are reported to measure the stability and performance of the model. 
Perturbation on the embedding space (radius $\delta_x=0.01$) are conducted on SST.}
\label{tab:ablation:main}
\vspace{-12pt}
\end{table}




==> SEAT_ Stable and Explainable Attention/tab/dataset.tex <==
\begin{table}[h]
    \centering
    \small
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cccc} 
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \textbf{Avg. Length} & \textbf{Train Size} & \textbf{Test Size}  \\ 
\cmidrule{2-4}
                         & (texts)     & (neg/pos)  & (neg/pos)  \\ 
\midrule
Emotion~                 & 91          & 1400/708   & 558/358    \\
SST~                     & 19          & 3610/3310  & 909/912    \\
Hate~                    & 23          & 3783/5217  & 1252/1718  \\
Rotten Tomatoes~         & 23          & 4265/4265  & 533/533    \\
\bottomrule
\end{tabular}
    }
    \caption{Dataset statistics. \label{tab:data}}
\end{table} 


==> SEAT_ Stable and Explainable Attention/tab/tab-abl-other3.tex <==
\begin{table}[htbp]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccc} 
\toprule
\multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Ablation Setting}} & \multicolumn{3}{c}{\textbf{Metrics}}                                                                                \\ 
\cmidrule(l){2-6}
                                 & $\mathcal{L}_3$ & $\mathcal{L}_{Topk}$        & \textbf{Comp.$\uparrow$}                                 & \textbf{Suff.$\downarrow$} & \textbf{Sens.$\downarrow$}  \\ 
\midrule
\multirow{4}{*}{\textbf{RNN}}    &                 &                             & 5.744                                                    & 7.02E-04                   & 0.090                       \\
                                 & $\rightt$       &                             & 5.280                                                    & 6.22E-04                   & 0.081                       \\
                                 &                 & $\rightt$                   & 5.944                                                    & 2.22E-04                   & 0.088                       \\
                                 & $\rightt$       & $\rightt$                   & \textbf{6.016}                                           & \textbf{1.02E-04}          & \textbf{0.076}              \\ 
\midrule
\multirow{4}{*}{\textbf{BiLSTM}} &                 &                             & 5.182                                                    & 0.255                      & 0.098                       \\
                                 & $\rightt$       &                             & 2.219                                                    & 0.016                      & 0.087                       \\
                                 &                 & $\rightt$                   & 5.167                                                    & 0.004                      & 0.095                       \\
                                 & $\rightt$       & $\rightt$                   & \begin{tabular}[c]{@{}c@{}}\textbf{5.435}\\\end{tabular} & \textbf{4.37E-06}          & \textbf{0.076}              \\ 
\midrule
\multirow{4}{*}{\textbf{BERT}}   &                 &                             & 0.003                                                    & 0.310                      & 0.009                       \\
                                 & $\rightt$       &                             & 0.002                                                    & 0.280                      & 0.005                       \\
                                 &                 & $\rightt$                   & 0.210                                                    & 0.090                      & 0.006                       \\
                                 & $\rightt$       & $\rightt$                   & \textbf{0.497}                                           & \textbf{0.019}             & \textbf{0.004}              \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of the proposed method on the explainability. We evaluate the effectiveness of the  the second term $\mathcal{L}_{Topk}$ and third term $\mathcal{L}_3$ in (\ref{eq:6}) on three different architectures. Comprehensiveness, Sufficiency and Sensitivity are reported to measure the explainability of the model. Here we conduct perturbation on the embedding space with radius of 0.01 on SST dataset.}
\label{tab:ablation-2}
\end{table}




==> SEAT_ Stable and Explainable Attention/tab/tab1.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{0.8}
\centering
% \small
\resizebox{1.0\linewidth}{!}{

\begin{tabular}{cccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}  & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Emotion}}                      & \multicolumn{3}{c}{\textbf{SST}}   & \multicolumn{3}{c}{\textbf{Hate}}  & \multicolumn{3}{c}{\textbf{RottenT}}  \\ 
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
                        &                         & \textbf{JSD$\downarrow$} & \textbf{TVD$\downarrow$} & \textbf{F1$\uparrow$} & \textbf{JSD}  & \textbf{TVD}  & \textbf{F1}  & \textbf{JSD}  & \textbf{TVD}  & \textbf{F1} & \textbf{JSD}  & \textbf{TVD}  & \textbf{F1}   \\ 
\midrule
\multirow{7}{*}{\textbf{RNN}}    & Vanilla                 & 0.002           & 20.145          & 0.663        & 0.019    & 19.566 & 0.811 & 0.009    & 15.576 & 0.553 & 0.008    & 19.139 & 0.763    \\
                        & Word-AT                 & 0.028           & 1.824           & 0.627        & 0.016    & 1.130  & 0.798 & 0.026    & 1.170  & 0.527 & 0.037    & 1.381  & 0.741    \\
                        & Word-iAT                & 0.042           & 2.691           & 0.653        & 0.023    & 1.277  & \textbf{0.815} & 0.022    & 1.049  & 0.523 & 0.054    & 1.336  & 0.766    \\
                        & Attention-RP            & 0.025           & 3.276           & 0.671        & 0.028    & 2.042  & 0.792 & 0.025    & 2.672  & 0.554 & 0.009    & 3.691  & \textbf{0.770}    \\
                        & Attention-AT            & 0.055           & 2.716           & 0.665        & 0.047    & 2.394  & 0.782 & 0.031    & 2.210  & 0.528 & 0.068    & 4.234  & 0.755    \\
                        & Attention-iAT           & 0.017           & 3.654           & 0.645        & 0.048    & 2.653  & 0.746 & 0.039    & 2.264  & 0.533 & 0.054    & 1.594  & 0.753    \\
                        \rowcolor{grey!20} & SEAT(\textbf{Ours})     & \textbf{3.81E-08}        & \textbf{1.750}           & \textbf{0.672}        & \textbf{2.75E-07} & \textbf{1.099}  & 0.813 & \textbf{1.79E-09} & \textbf{0.908}  & \textbf{0.579} & \textbf{6.46E-07} & \textbf{1.178}  & 0.763    \\ 
\midrule
\midrule
\multirow{7}{*}{\textbf{BiLSTM}} & Vanilla                 & 0.002           & 23.447          & 0.612        & 0.027    & 18.640 & \textbf{0.809} & 0.060    & 15.633 & 0.524 & 0.009    & 20.125 & 0.764    \\
                        & Word-AT                 & 0.050           & 1.927           & 0.662        & 0.020    & 0.810  & 0.798 & 0.084    & 1.537  & 0.538 & 0.031    & 1.071  & 0.757    \\
                        & Word-iAT                & 0.058           & 1.139           & 0.640        & 0.034    & 1.037  & 0.802 & 0.091    & 1.590  & 0.530 & 0.045    & 1.218  & 0.765    \\
                        & Attention-RP            & 0.031           & 1.326           & 0.642        & 0.034    & 1.267  & 0.772 & 0.052    & 1.299  & 0.522 & 0.066    & 1.412  & 0.764    \\
                        & Attention-AT            & 0.076           & 1.541           & \textbf{0.672}        & 0.028    & 1.661  & 0.779 & 0.057    & 1.504  & 0.523 & 0.079    & 2.044  & 0.766    \\
                        & Attention-iAT           & 0.033           & 1.267           & 0.651        & 0.034    & 1.528  & 0.801 & 0.062    & 2.256  & 0.525 & 0.076    & 1.751  & \textbf{0.777}    \\
                        \rowcolor{grey!20} &  SEAT(\textbf{Ours})     & \textbf{1.23E-08}  & \textbf{0.736}           & 0.670        & \textbf{1.80E-08} & \textbf{0.777}  & 0.802 & \textbf{8.49E-09} & \textbf{1.030}  & \textbf{0.543} & \textbf{2.57E-08} & \textbf{0.885}  & 0.771    \\ 
\midrule
\midrule
\multirow{7}{*}{\textbf{BERT}}   & Vanilla                 & 0.024           & 2.127           & \textbf{0.721}        & 0.005    & 2.605  & 0.912 & 0.036    & 1.771  & 0.493 & 0.010    & 2.500  & \textbf{0.845}    \\
                        & Word-AT                 & 0.085           & 0.060           & 0.694        & 0.267    & 0.055  & 0.900 & 0.170    & 0.043  & \textbf{0.554} & 0.510    & 0.036  & 0.826    \\
                        & Word-iAT                & 0.584           & 0.029           & 0.694        & 0.241    & 0.054  & 0.895 & 0.166    & 0.049  & 0.496 & 0.480    & 0.049  & 0.844    \\
                        & Attention-RP            & 0.035           & 0.232           & 0.657        & 0.086    & 0.127  & 0.893 & 0.079    & 0.277  & \textbf{0.554} & 0.078    & 0.142  & 0.817    \\
                        & Attention-AT            & 0.067           & 0.119           & 0.707        & 0.005    & 0.156  & 0.907 & 0.031    & 0.230  & 0.510 & 0.041    & 0.189  & 0.818    \\
                        & Attention-iAT           & 0.096           & 0.222           & 0.684        & 0.129    & 0.200  & \textbf{0.915} & 0.074    & 0.271  & 0.512 & 0.108    & 0.183  & 0.831    \\
                        \rowcolor{grey!20} &  SEAT(\textbf{Ours})     & \textbf{4.70E-07}        & \textbf{0.002}           & 0.713        & \textbf{2.77E-07} & \textbf{0.036}  & 0.907 & \textbf{2.42E-06} & \textbf{0.042}  & 0.545 & \textbf{1.68E-08} & \textbf{0.003}  & 0.841   \\
\bottomrule
\end{tabular}
}
\caption{Results of evaluating embedding perturbation stability of (modified) attentions given by different methods using RNN, BiLSTM, and BERT under three metrics (JSD is for attention weight distribution, TVD is for output distribution, and F1 score is for model performance). The perturbation radius is set as $\delta_x$=1e-3. $\uparrow$ means a higher value under this metric indicates better results, and $\downarrow$ means the opposite. The best performance is \textbf{bolded}. Same symbols are used in the following tables by default. \label{golden}}
\end{table*}


==> SEAT_ Stable and Explainable Attention/tab/tab2.tex <==
\vspace{-10pt}
\begin{table*}[!ht]
\renewcommand{\arraystretch}{0.8}
\centering
% \small
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccccccccccc} 
\toprule
\multirow{2}{*}{\textbf{Model}}  & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{IMDB}}                                                                         & \multicolumn{3}{c}{\textbf{SST}}     & \multicolumn{3}{c}{\textbf{Hate}}    & \multicolumn{3}{c}{\textbf{RottenT}}  \\ 
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(r){12-14}
                        &    & \textbf{Comp.$\uparrow$} & \textbf{Suff.$\downarrow$} & \textbf{Sens.$\downarrow$} & \textbf{Comp.}    & \textbf{Suff.}    & \textbf{Sens.} & \textbf{Comp.}    & \textbf{Suff.}    & \textbf{Sens.} & \textbf{Comp.}    & \textbf{Suff.} & \textbf{Sens.}     \\ 
\midrule
\multirow{7}{*}{\textbf{RNN}}    & Vanilla                 & 0.004                          & 0.007                          & 0.131                          & 5.744    & 7.02E-04 & 0.090 & 0.009    & 0.066    & 0.138 & 4.483    & 0.026 & 0.090     \\
                        & Word-AT                 & 2.899                          & 0.018                          & 0.121                          & 5.280    & \textbf{0.000} & 0.081 & 2.408    & 0.058    & 0.137 & 2.512    & 0.031 & 0.093     \\
                        & Word-iAT                & 2.060                          & 0.010                          & 0.122                          & 5.452    & 9.35E-06 & 0.121 & 6.069    & 0.075    & 0.136 & 4.534    & 0.058 & 0.087     \\
                        & Attention-RP            & 0.099                          & 0.073                          & 0.130                          & 6.001    & 2.87E-04 & 0.085 & 3.585    & 0.080    & 0.133 & 4.637    & 0.052 & 0.094     \\
                        & Attention-AT            & 0.026                          & 0.052                          & 0.131                          & 3.118    & \textbf{0.000} & 0.088 & 2.493    & 0.372    & 0.134 & 4.713    & 0.049 & 0.096     \\
                        & Attention-iAT           & 1.994                          & 6.74E-04                       & 0.117                          & 4.788    & \textbf{0.000} & 0.091 & 5.351    & 0.126    & 0.133 & 2.435    & 0.039 & 0.086     \\
                        \rowcolor{grey!20} &  SEAT(\textbf{Ours})     & \textbf{3.281}                          & \textbf{1.04E-05}                       & \textbf{0.106}                          & \textbf{6.016}    & \textbf{0.000} & \textbf{0.076} & \textbf{6.558}    & \textbf{2.75E-04} & \textbf{0.129} & \textbf{4.796}    & \textbf{0.025} & \textbf{0.084}     \\ 
\midrule
\midrule
\multirow{7}{*}{\textbf{BiLSTM}} & Vanilla                 & 0.474                          & 0.002                          & 0.129                          & 5.182    & 0.255    & 0.086 & 4.203    & 0.112    & 0.142 & 2.966    & 0.088 & 0.092     \\
                        & Word-AT                 & 1.449                          & 0.015                          & 0.121                          & 5.167    & 8.44E-04 & 0.096 & 5.438    & 0.207    & 0.153 & 3.388    & 0.062 & 0.080     \\
                        & Word-iAT                & 0.619                          & 0.005                          & 0.127                          & 5.259    & 3.81E-05 & 0.087 & 4.568    & 0.320    & 0.145 & 3.339    & 0.078 & 0.082     \\
                        & Attention-RP            & 0.561                          & 0.002                          & 0.127                          & 2.865    & 0.007    & 0.101 & 2.248    & 0.199    & 0.148 & 4.073    & 0.200 & 0.082     \\
                        & Attention-AT            & 1.294                          & 0.051                          & 0.111                          & 2.129    & 0.004    & 0.098 & 3.220    & 0.065    & \textbf{0.140} & 4.925    & 0.216 & 0.082     \\
                        & Attention-iAT           & 0.555                          & 0.002                          & 0.127                          & 5.176    & 0.004    & 0.083 & 4.092    & 0.290    & 0.141 & 2.431    & 0.377 & 0.083     \\
                        \rowcolor{grey!20} &  SEAT(\textbf{Ours})     & \textbf{1.502}                          & \textbf{6.41E-04}                       & \textbf{0.098}                          & \textbf{5.435}    & \textbf{4.37E-06} & \textbf{0.076} & \textbf{6.240}    & \textbf{0.025}    & \textbf{0.140} & \textbf{4.941}    & \textbf{0.046} & \textbf{0.077}     \\ 
\midrule
\midrule
\multirow{7}{*}{\textbf{BERT}}   & Vanilla                 & 5.07E-04                       & 0.008                          & 0.013                          & 0.003    & 0.310    & 0.009 & 3.20E-04 & 0.401    & 0.016 & 0.001    & 0.092 & 0.010     \\
                        & Word-AT                 & 5.01E-05                       & 0.005                          & 0.016                          & 1.26E-05 & 4.47E-04 & 0.005 & 4.01E-04 & 0.014    & 0.017 & 0.005    & 0.043 & 0.016     \\
                        & Word-iAT                & 5.47E-04                       & 0.007                          & 0.017                          & 1.51E-05 & 5.67E-04 & 0.004 & 0.003    & 0.045    & 0.017 & 2.93E-04 & 0.010 & 0.009     \\
                        & Attention-RP            & 0.085                          & 0.086                          & 0.014                          & 0.002    & 0.010    & 0.011 & 0.035    & 0.034    & 0.016 & 0.017    & 0.003 & 0.010     \\
                        & Attention-AT            & 4.65E-05                       & 0.338                          & 0.016                          & 4.50E-05 & 0.441    & 0.006 & \textbf{0.004}    & 0.007    & 0.016 & 6.26E-04 & 0.032 & 0.011     \\
                        & Attention-iAT           & 0.002                          & 0.164                          & 0.015                          & 1.19E-04 & 9.07E-04 & 0.007 & 0.001    & 0.151    & 0.017 & 0.003    & 0.025 & 0.010     \\
                        \rowcolor{grey!20} & SEAT(\textbf{Ours})     & \textbf{0.160}                          & \textbf{0.002}                          & \textbf{0.012}                          & \textbf{0.497}    & \textbf{0.000} & \textbf{0.004} & \textbf{0.153}    & \textbf{0.006}    & \textbf{0.015} & \textbf{0.040}    & \textbf{0.002} & \textbf{0.008}     \\
\bottomrule
\end{tabular}
}
\caption{Results on evaluating the interpretability of different methods. We conduct experiments with three architectures, including RNN, BiLSTM, and BERT, under three criteria (comprehensiveness, sufficiency, and sensitivity score) on text classification datasets. The best performance is \textbf{bolded}.}
\label{golden-explanation}
\vspace{-12pt}
\end{table*}


==> SEAT_ Stable and Explainable Attention/tab/tab3.tex <==
\begin{table*}[ht]
\small
% \resizebox{}{}{}
\centering
\label{tab:diff_rad}
% \footnotesize
% \scriptsize
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|cccccccccccccc} 
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Radius($\delta_x$)}} & \multirow{2}{*}{Model}  & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Emotion}                                                             & \multicolumn{3}{c}{SST}   & \multicolumn{3}{c}{Hate}  & \multicolumn{3}{c}{RottenT}   \\ 
\cmidrule(r){4-6}\cmidrule(r){7-9}\cmidrule(r){10-12}\cmidrule(lr){13-15}
\multicolumn{1}{c}{}                                                        &                         &                         & JSD$\downarrow$ & TVD$\downarrow$ & F1$\uparrow$ & JSD      & TVD    & F1    & JSD      & TVD    & F1    & JSD       & TVD      & F1     \\ 
\midrule
\multirow{21}{*}{0.005}                                                     & \multirow{7}{*}{RNN}    & Vanilla                 & 0.002                        & 20.120                       & 0.677                     & 0.019    & 19.916 & 0.767 & 0.009    & 15.627 & 0.513 & 0.008     & 19.240   & 0.763  \\
                                                                            &                         & Word-AT                 & 0.016                        & 1.634                        & 0.642                     & 0.017    & 2.186  & 0.800 & 0.035    & 1.618  & 0.519 & 0.058     & 1.401    & 0.768  \\
                                                                            &                         & Word-iAT                & 0.027                        & 1.570                        & 0.637                     & 0.021    & 1.331  & 0.811 & 0.025    & 1.387  & 0.537 & 0.092     & 1.719    & 0.759  \\
                                                                            &                         & Attention-RP            & 0.026                        & 3.281                        & 0.671                     & 0.028    & 2.209  & 0.792 & 0.025    & 2.650  & 0.554 & 0.009     & 3.759    & 0.770  \\
                                                                            &                         & Attention-AT            & 0.055                        & 2.738                        & 0.665                     & 0.047    & 2.595  & 0.782 & 0.032    & 2.195  & 0.528 & 0.068     & 4.328    & 0.755  \\
                                                                            &                         & Attention-iAT           & 0.017                        & 3.573                        & 0.645                     & 0.050    & 2.821  & 0.746 & 0.039    & 2.261  & 0.533 & 0.055     & 1.645    & 0.753  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 8.41E-09                     & 1.320                        & 0.689                     & 4.19E-08 & 1.143  & 0.803 & 2.51E-09 & 1.263  & 0.579 & -2.87E-10 & 1.174    & 0.762  \\ 
\cmidrule{2-15}
                                                                            & \multirow{7}{*}{BiLSTM} & Vanilla                 & 0.002                        & 23.440                       & 0.653                     & 0.037    & 19.215 & 0.809 & 0.062    & 15.805 & 0.524 & 0.009     & 20.197   & 0.764  \\
                                                                            &                         & Word-AT                 & 0.053                        & 1.632                        & 0.655                     & 0.025    & 1.080  & 0.794 & 0.058    & 2.126  & 0.528 & 0.039     & 1.223    & 0.772  \\
                                                                            &                         & Word-iAT                & 0.054                        & 1.902                        & 0.643                     & 0.029    & 1.120  & 0.809 & 0.078    & 1.899  & 0.525 & 0.064     & 1.187    & 0.750  \\
                                                                            &                         & Attention-RP            & 0.031                        & 1.391                        & 0.642                     & 0.036    & 1.396  & 0.772 & 0.054    & 1.388  & 0.522 & 0.068     & 1.539    & 0.764  \\
                                                                            &                         & Attention-AT            & 0.079                        & 1.617                        & 0.672                     & 0.030    & 1.748  & 0.779 & 0.058    & 1.582  & 0.523 & 0.080     & 2.129    & 0.766  \\
                                                                            &                         & Attention-iAT           & 0.035                        & 1.371                        & 0.651                     & 0.036    & 1.722  & 0.801 & 0.063    & 2.310  & 0.525 & 0.079     & 1.931    & 0.777  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 9.68E-09                     & 0.736                        & 0.671                     & 2.70E-08 & 1.040  & 0.805 & 1.47E-08 & 1.081  & 0.543 & 2.06E-08  & 0.991    & 0.770  \\ 
\cmidrule{2-15}
                                                                            & \multirow{7}{*}{BERT}   & Vanilla                 & 0.026                        & 2.130                        & 0.721                     & 0.004    & 2.610  & 0.912 & 0.039    & 1.771  & 0.493 & 0.010     & 2.504    & 0.845  \\
                                                                            &                         & Word-AT                 & 0.013                        & 0.024                        & 0.694                     & 0.100    & 0.035  & 0.891 & 0.006    & 0.074  & 0.579 & 0.563     & 0.083    & 0.845  \\
                                                                            &                         & Word-iAT                & 0.456                        & 0.059                        & 0.658                     & 0.213    & 0.094  & 0.912 & 0.331    & 0.043  & 0.501 & 0.488     & 0.048    & 0.852  \\
                                                                            &                         & Attention-RP            & 0.039                        & 0.235                        & 0.657                     & 0.089    & 0.128  & 0.893 & 0.085    & 0.278  & 0.554 & 0.078     & 0.143    & 0.817  \\
                                                                            &                         & Attention-AT            & 0.081                        & 0.019                        & 0.707                     & 0.006    & 0.157  & 0.907 & 0.035    & 0.230  & 0.510 & 0.049     & 0.193    & 0.818  \\
                                                                            &                         & Attention-iAT           & 0.126                        & 0.228                        & 0.684                     & 0.147    & 0.204  & 0.915 & 0.080    & 0.271  & 0.512 & 0.135     & 0.187    & 0.831  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 1.70E-08                     & 0.001                        & 0.717                     & 1.29E-07 & 0.028  & 0.911 & 6.47E-06 & 0.003  & 0.575 & 2.61E-05  & 0.033    & 0.848  \\ 
\midrule
\multirow{21}{*}{0.01}                                                      & \multirow{7}{*}{RNN}    & Vanilla                 & 0.002                        & 20.119                       & 0.657                     & 0.021    & 20.716 & 0.797 & 0.010    & 15.798 & 0.513 & 0.008     & 19.383   & 0.763  \\
                                                                            &                         & Word-AT                 & 0.017                        & 1.385                        & 0.629                     & 0.017    & 1.266  & 0.814 & 0.023    & 1.238  & 0.532 & 0.054     & 1.196    & 0.765  \\
                                                                            &                         & Word-iAT                & 0.027                        & 1.576                        & 0.637                     & 0.021    & 1.331  & 0.811 & 0.025    & 1.248  & 0.537 & 0.092     & 1.716    & 0.759  \\
                                                                            &                         & Attention-RP            & 0.026                        & 3.296                        & 0.671                     & 0.028    & 2.208  & 0.792 & 0.025    & 2.662  & 0.554 & 0.009     & 3.750    & 0.770  \\
                                                                            &                         & Attention-AT            & 0.055                        & 2.717                        & 0.665                     & 0.048    & 2.587  & 0.782 & 0.032    & 2.209  & 0.528 & 0.068     & 4.358    & 0.755  \\
                                                                            &                         & Attention-iAT           & 0.017                        & 3.554                        & 0.645                     & 0.050    & 2.837  & 0.746 & 0.039    & 2.261  & 0.533 & 0.055     & 1.646    & 0.753  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 1.40E-08                     & 1.250                        & 0.688                     & 6.44E-08 & 1.175  & 0.813 & 6.48E-10 & 1.198  & 0.579 & 1.16E-07  & 0.975    & 0.762  \\ 
\cmidrule{2-15}
                                                                            & \multirow{7}{*}{BiLSTM} & Vanilla                 & 0.002                        & 23.432                       & 0.643                     & 0.059    & 20.398 & 0.809 & 0.072    & 16.312 & 0.524 & 0.010     & 20.322   & 0.764  \\
                                                                            &                         & Word-AT                 & 0.045                        & 1.551                        & 0.658                     & 0.033    & 1.214  & 0.802 & 0.071    & 1.609  & 0.516 & 0.062     & 1.214    & 0.765  \\
                                                                            &                         & Word-iAT                & 0.054                        & 1.899                        & 0.643                     & 0.029    & 1.594  & 0.809 & 0.078    & 1.899  & 0.525 & 0.064     & 1.203    & 0.750  \\
                                                                            &                         & Attention-RP            & 0.031                        & 1.390                        & 0.642                     & 0.036    & 1.398  & 0.772 & 0.054    & 1.386  & 0.522 & 0.068     & 1.540    & 0.764  \\
                                                                            &                         & Attention-AT            & 0.080                        & 1.613                        & 0.672                     & 0.030    & 1.745  & 0.779 & 0.058    & 1.581  & 0.523 & 0.080     & 2.130    & 0.766  \\
                                                                            &                         & Attention-iAT           & 0.035                        & 1.370                        & 0.651                     & 0.036    & 1.724  & 0.801 & 0.063    & 2.315  & 0.525 & 0.079     & 1.932    & 0.777  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 1.04E-08                     & 0.960                        & 0.664                     & 1.63E-07 & 1.116  & 0.804 & 8.17E-09 & 1.167  & 0.547 & 6.44E-09  & 0.948    & 0.770  \\ 
\cmidrule{2-15}
                                                                            & \multirow{7}{*}{BERT}   & Vanilla                 & 0.033                        & 2.134                        & 0.721                     & 0.004    & 2.617  & 0.912 & 0.047    & 1.772  & 0.493 & 0.010     & 2.508    & 0.845  \\
                                                                            &                         & Word-AT                 & 0.004                        & 0.040                        & 0.694                     & 0.118    & 0.046  & 0.909 & 0.309    & 0.074  & 0.540 & 0.390     & 0.086    & 0.829  \\
                                                                            &                         & Word-iAT                & 0.456                        & 0.059                        & 0.658                     & 0.213    & 0.107  & 0.912 & 0.331    & 0.100  & 0.501 & 0.488     & 0.048    & 0.852  \\
                                                                            &                         & Attention-RP            & 0.039                        & 0.235                        & 0.657                     & 0.089    & 0.128  & 0.893 & 0.085    & 0.278  & 0.554 & 0.078     & 0.143    & 0.817  \\
                                                                            &                         & Attention-AT            & 0.082                        & 0.025                        & 0.707                     & 0.006    & 0.157  & 0.907 & 0.035    & 0.230  & 0.510 & 0.049     & 0.193    & 0.818  \\
                                                                            &                         & Attention-iAT           & 0.126                        & 0.228                        & 0.684                     & 0.147    & 0.204  & 0.915 & 0.081    & 0.271  & 0.512 & 0.135     & 0.187    & 0.831  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 3.61E-09                     & 0.001                        & 0.713                     & 2.49E-07 & 0.028  & 0.909 & 8.38E-06 & 0.044  & 0.561 & 1.18E-06  & 0.034    & 0.844  \\ 
\midrule
\multirow{21}{*}{0.05}                                                      & \multirow{7}{*}{RNN}    & Vanilla                 & 0.006                        & 20.911                       & 0.667                     & 0.047    & 28.278 & 0.767 & 0.025    & 18.398 & 0.513 & 0.015     & 21.265   & 0.763  \\
                                                                            &                         & Word-AT                 & 0.023                        & 1.652                        & 0.627                     & 0.019    & 1.270  & 0.797 & 0.031    & 1.320  & 0.522 & 0.030     & 1.126    & 0.748  \\
                                                                            &                         & Word-iAT                & 0.027                        & 1.577                        & 0.637                     & 0.021    & 1.325  & 0.811 & 0.025    & 1.235  & 0.537 & 0.092     & 1.704    & 0.759  \\
                                                                            &                         & Attention-RP            & 0.026                        & 3.294                        & 0.671                     & 0.028    & 2.212  & 0.792 & 0.025    & 2.662  & 0.554 & 0.009     & 3.763    & 0.770  \\
                                                                            &                         & Attention-AT            & 0.055                        & 2.675                        & 0.665                     & 0.048    & 2.611  & 0.782 & 0.032    & 2.210  & 0.528 & 0.068     & 4.370    & 0.755  \\
                                                                            &                         & Attention-iAT           & 0.017                        & 3.559                        & 0.645                     & 0.050    & 2.814  & 0.746 & 0.039    & 2.277  & 0.533 & 0.055     & 1.634    & 0.753  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 1.87E-08                     & 1.546                        & 0.691                     & 3.77E-08 & 1.098  & 0.805 & 4.54E-10 & 1.213  & 0.579 & -3.39E-11 & 3.02E-04 & 0.767  \\ 
\cmidrule{2-15}
                                                                            & \multirow{7}{*}{BiLSTM} & Vanilla                 & 0.003                        & 23.377                       & 0.653                     & 0.258    & 28.472 & 0.809 & 0.190    & 20.458 & 0.524 & 0.022     & 22.146   & 0.764  \\
                                                                            &                         & Word-AT                 & 0.022                        & 1.279                        & 0.656                     & 0.028    & 1.062  & 0.790 & 0.055    & 1.771  & 0.521 & 0.047     & 1.451    & 0.769  \\
                                                                            &                         & Word-iAT                & 0.054                        & 1.900                        & 0.643                     & 0.029    & 1.109  & 0.809 & 0.077    & 1.862  & 0.525 & 0.063     & 1.194    & 0.750  \\
                                                                            &                         & Attention-RP            & 0.031                        & 1.390                        & 0.642                     & 0.036    & 1.409  & 0.772 & 0.054    & 1.381  & 0.522 & 0.067     & 1.533    & 0.764  \\
                                                                            &                         & Attention-AT            & 0.080                        & 1.622                        & 0.672                     & 0.030    & 1.745  & 0.779 & 0.058    & 1.572  & 0.523 & 0.080     & 2.126    & 0.766  \\
                                                                            &                         & Attention-iAT           & 0.035                        & 1.368                        & 0.651                     & 0.036    & 1.712  & 0.801 & 0.063    & 2.314  & 0.525 & 0.078     & 1.907    & 0.777  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 1.44E-08                     & 1.094                        & 0.664                     & 1.04E-08 & 1.043  & 0.801 & 1.47E-08 & 1.229  & 0.524 & 1.35E-08  & 1.027    & 0.768  \\ 
\cmidrule{2-15}
                                                                            & \multirow{7}{*}{BERT}   & Vanilla                 & 0.193                        & 2.197                        & 0.721                     & 0.008    & 2.680  & 0.912 & 0.193    & 1.780  & 0.493 & 0.042     & 2.553    & 0.845  \\
                                                                            &                         & Word-AT                 & 0.004                        & 0.022                        & 0.694                     & 0.175    & 0.065  & 0.910 & 0.111    & 0.058  & 0.546 & 0.473     & 0.056    & 0.836  \\
                                                                            &                         & Word-iAT                & 0.456                        & 0.059                        & 0.658                     & 0.213    & 0.046  & 0.912 & 0.331    & 0.044  & 0.501 & 0.488     & 0.048    & 0.852  \\
                                                                            &                         & Attention-RP            & 0.039                        & 0.235                        & 0.657                     & 0.089    & 0.128  & 0.893 & 0.085    & 0.278  & 0.554 & 0.078     & 0.143    & 0.817  \\
                                                                            &                         & Attention-AT            & 0.082                        & 0.003                        & 0.707                     & 0.006    & 0.157  & 0.907 & 0.035    & 0.230  & 0.510 & 0.049     & 0.193    & 0.818  \\
                                                                            &                         & Attention-iAT           & 0.126                        & 0.228                        & 0.684                     & 0.147    & 0.204  & 0.915 & 0.081    & 0.271  & 0.512 & 0.136     & 0.187    & 0.831  \\
                                                                            &                         & SEAT(\textbf{Ours})     & 1.72E-09                     & 0.001                        & 0.717                     & 1.55E-06 & 0.028  & 0.910 & 8.69E-06 & 0.037  & 0.555 & 1.10E-05  & 0.035    & 0.849  \\
\bottomrule
\end{tabular}
}
\caption{More results on the performance of different methods under different perturbation radii. JSD and TVD are reported to measure the stability while F1 measure the model accuracy of the clean data. From the table we can see that SEAT have lower JSD and TVD with little or even no drop for F1 under all the settings. These suggest that our method suppresses other baseline methods on both model stability and effectiveness. \label{tab: more result main 3 metrics}}
\end{table*} 



==> SEAT_ Stable and Explainable Attention/tab/tab4.tex <==
\begin{table*}[ht]
\small
% \resizebox{}{}{}
\centering
% \label{tab:}
% \footnotesize
% \scriptsize
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|cccccccccccccc} 
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Radius($\delta_{x}$)}} & \multirow{2}{*}{Model}  & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Emotion}                             & \multicolumn{3}{c}{SST}     & \multicolumn{3}{c}{Hate}    & \multicolumn{3}{c}{RottenT}  \\ 
\cmidrule(l){4-15}
\multicolumn{1}{c}{}                                    &                         &                         & Comp.$\uparrow$ & Suff.$\downarrow$ & Sens.$\downarrow$ & Comp.    & Suff.    & Sens. & Comp.    & Suff.    & Sens. & Comp.    & Suff.    & Sens.  \\ 
\midrule
\multirow{21}{*}{0.005}                                 & \multirow{7}{*}{RNN}    & Vanilla                 & 3.281           & 0.007             & 0.143             & 5.744    & 3.90E-04 & 0.160 & 0.073    & 0.066    & 0.179 & 4.483    & 0.127    & 0.120  \\
                                                        &                         & Word-AT                 & 0.006           & 0.072             & 0.149             & 5.585    & 0.00E+00 & 0.157 & 3.259    & 0.246    & 0.198 & 2.744    & 0.255    & 0.113  \\
                                                        &                         & Word-iAT                & 0.365           & 0.005             & 0.139             & 4.433    & 5.85E-04 & 0.155 & 2.178    & 0.091    & 0.174 & 2.804    & 0.091    & 0.122  \\
                                                        &                         & Attention-RP            & 0.099           & 0.073             & 0.133             & 6.001    & 2.87E-04 & 0.144 & 3.585    & 0.080    & 0.169 & 4.637    & 0.052    & 0.127  \\
                                                        &                         & Attention-AT            & 0.026           & 0.052             & 0.132             & 5.608    & 0.00E+00 & 0.144 & 2.493    & 0.372    & 0.172 & 4.713    & 0.049    & 0.128  \\
                                                        &                         & Attention-iAT           & 1.994           & 6.74E-04          & 0.138             & 4.788    & 0.00E+00 & 0.159 & 5.351    & 0.126    & 0.179 & 2.435    & 0.039    & 0.119  \\
                                                        &                         & SEAT(\textbf{Ours})     & 5.099           & 1.74E-05          & 0.131             & 6.016    & 0.00E+00 & 0.140 & 6.558    & 0.001    & 0.131 & 5.342    & 0.026    & 0.105  \\ 
\cmidrule{2-15}
                                                        & \multirow{7}{*}{BiLSTM} & Vanilla                 & 0.474           & 0.002             & 0.136             & 5.182    & 0.003    & 0.147 & 4.795    & 0.112    & 0.199 & 2.966    & 0.088    & 0.125  \\
                                                        &                         & Word-AT                 & 2.195           & 0.029             & 0.193             & 2.783    & 0.007    & 0.155 & 3.085    & 0.111    & 0.188 & 1.827    & 0.117    & 0.135  \\
                                                        &                         & Word-iAT                & 1.765           & 0.015             & 0.190             & 5.082    & 2.62E-04 & 0.165 & 5.409    & 0.093    & 0.202 & 3.759    & 0.100    & 0.119  \\
                                                        &                         & Attention-RP            & 0.561           & 0.002             & 0.173             & 2.865    & 0.007    & 0.149 & 2.248    & 0.199    & 0.189 & 4.073    & 0.200    & 0.117  \\
                                                        &                         & Attention-AT            & 1.294           & 6.41E-04          & 0.143             & 2.129    & 0.004    & 0.129 & 3.220    & 0.124    & 0.190 & 4.925    & 0.216    & 0.122  \\
                                                        &                         & Attention-iAT           & 0.555           & 0.002             & 0.135             & 5.435    & 0.004    & 0.152 & 4.092    & 0.290    & 0.197 & 4.941    & 0.377    & 0.143  \\
                                                        &                         & SEAT(\textbf{Ours})     & 2.306           & 4.45E-04          & 0.135             & 5.454    & 4.37E-06 & 0.129 & 6.240    & 0.065    & 0.187 & 4.956    & 0.037    & 0.114  \\ 
\cmidrule{2-15}
                                                        & \multirow{7}{*}{BERT}   & Vanilla                 & 5.07E-04        & 0.008             & 0.016             & 0.003    & 0.310    & 0.010 & 3.20E-04 & 0.006    & 0.017 & 0.001    & 0.092    & 0.010  \\
                                                        &                         & Word-AT                 & 6.44E-05        & 0.014             & 0.016             & 0.164    & 0.165    & 0.007 & 4.09E-06 & 0.012    & 0.018 & 4.82E-04 & 0.005    & 0.011  \\
                                                        &                         & Word-iAT                & 4.79E-04        & 0.013             & 0.016             & 9.51E-04 & 0.024    & 0.008 & 3.80E-04 & 0.012    & 0.019 & 6.15E-04 & 0.016    & 0.012  \\
                                                        &                         & Attention-RP            & 0.085           & 0.086             & 0.015             & 0.002    & 0.010    & 0.012 & 0.035    & 0.034    & 0.018 & 0.017    & 0.003    & 0.010  \\
                                                        &                         & Attention-AT            & 4.65E-05        & 0.003             & 0.017             & 5.82E-04 & 0.450    & 0.007 & 0.004    & 0.007    & 0.017 & 0.001    & 0.116    & 0.011  \\
                                                        &                         & Attention-iAT           & 5.74E-05        & 0.164             & 0.016             & 1.19E-04 & 9.07E-04 & 0.007 & 4.05E-04 & 0.151    & 0.017 & 0.003    & 0.025    & 0.011  \\
                                                        &                         & SEAT(\textbf{Ours})     & 0.160           & 0.002             & 0.014             & 0.497    & 0.00E+00 & 0.007 & 0.153    & 6.74E-05 & 0.016 & 0.040    & 0.002    & 0.009  \\ 
\midrule
\multirow{21}{*}{0.01}                                  & \multirow{7}{*}{RNN}    & Vanilla                 & 0.004           & 0.007             & 0.131             & 5.744    & 7.02E-04 & 0.090 & 0.009    & 0.066    & 0.138 & 4.483    & 0.026    & 0.090  \\
                                                        &                         & Word-AT                 & 2.899           & 0.018             & 0.121             & 5.280    & 0.00E+00 & 0.081 & 2.408    & 0.058    & 0.137 & 2.512    & 0.031    & 0.093  \\
                                                        &                         & Word-iAT                & 2.060           & 0.010             & 0.122             & 5.452    & 9.35E-06 & 0.121 & 6.069    & 0.075    & 0.136 & 4.534    & 0.058    & 0.087  \\
                                                        &                         & Attention-RP            & 0.099           & 0.073             & 0.130             & 6.001    & 2.87E-04 & 0.085 & 3.585    & 0.080    & 0.133 & 4.637    & 0.052    & 0.094  \\
                                                        &                         & Attention-AT            & 0.026           & 0.052             & 0.131             & 3.118    & 0.00E+00 & 0.088 & 2.493    & 0.372    & 0.134 & 4.713    & 0.049    & 0.096  \\
                                                        &                         & Attention-iAT           & 1.994           & 6.74E-04          & 0.117             & 4.788    & 0.00E+00 & 0.091 & 5.351    & 0.126    & 0.133 & 2.435    & 0.039    & 0.086  \\
                                                        &                         & SEAT(\textbf{Ours})     & 3.281           & 1.04E-05          & 0.106             & 6.016    & 0.00E+00 & 0.076 & 6.558    & 2.75E-04 & 0.129 & 4.796    & 0.025    & 0.084  \\ 
\cmidrule{2-15}
                                                        & \multirow{7}{*}{BiLSTM} & Vanilla                 & 0.474           & 0.002             & 0.129             & 5.182    & 0.255    & 0.086 & 4.203    & 0.112    & 0.142 & 2.966    & 0.088    & 0.092  \\
                                                        &                         & Word-AT                 & 1.449           & 0.015             & 0.121             & 5.167    & 8.44E-04 & 0.096 & 5.438    & 0.207    & 0.153 & 3.388    & 0.062    & 0.080  \\
                                                        &                         & Word-iAT                & 0.619           & 0.005             & 0.127             & 5.259    & 3.81E-05 & 0.087 & 4.568    & 0.320    & 0.145 & 3.339    & 0.078    & 0.082  \\
                                                        &                         & Attention-RP            & 0.561           & 0.002             & 0.127             & 2.865    & 0.007    & 0.101 & 2.248    & 0.199    & 0.148 & 4.073    & 0.200    & 0.082  \\
                                                        &                         & Attention-AT            & 1.294           & 0.051             & 0.111             & 2.129    & 0.004    & 0.098 & 3.220    & 0.065    & 0.140 & 4.925    & 0.216    & 0.082  \\
                                                        &                         & Attention-iAT           & 0.555           & 0.002             & 0.127             & 5.176    & 0.004    & 0.083 & 4.092    & 0.290    & 0.141 & 2.431    & 0.377    & 0.083  \\
                                                        &                         & SEAT(\textbf{Ours})     & 1.502           & 6.41E-04          & 0.098             & 5.435    & 4.37E-06 & 0.076 & 6.240    & 0.025    & 0.140 & 4.941    & 0.046    & 0.077  \\ 
\cmidrule{2-15}
                                                        & \multirow{7}{*}{BERT}   & Vanilla                 & 5.07E-04        & 0.008             & 0.013             & 0.003    & 0.310    & 0.009 & 3.20E-04 & 0.401    & 0.016 & 0.001    & 0.092    & 0.010  \\
                                                        &                         & Word-AT                 & 5.01E-05        & 0.005             & 0.016             & 1.26E-05 & 4.47E-04 & 0.005 & 4.01E-04 & 0.014    & 0.017 & 0.005    & 0.043    & 0.016  \\
                                                        &                         & Word-iAT                & 5.47E-04        & 0.007             & 0.017             & 1.51E-05 & 5.67E-04 & 0.004 & 0.003    & 0.045    & 0.017 & 2.93E-04 & 0.010    & 0.009  \\
                                                        &                         & Attention-RP            & 0.085           & 0.086             & 0.014             & 0.002    & 0.010    & 0.011 & 0.035    & 0.034    & 0.016 & 0.017    & 0.003    & 0.010  \\
                                                        &                         & Attention-AT            & 4.65E-05        & 0.338             & 0.016             & 4.50E-05 & 0.441    & 0.006 & 0.004    & 0.007    & 0.016 & 6.26E-04 & 0.032    & 0.011  \\
                                                        &                         & Attention-iAT           & 0.002           & 0.164             & 0.015             & 1.19E-04 & 9.07E-04 & 0.007 & 0.001    & 0.151    & 0.017 & 0.003    & 0.025    & 0.010  \\
                                                        &                         & SEAT(\textbf{Ours})     & 0.160           & 0.002             & 0.012             & 0.497    & 0.00E+00 & 0.004 & 0.153    & 0.006    & 0.015 & 0.040    & 0.002    & 0.008  \\ 
\midrule
\multirow{21}{*}{0.05}                                  & \multirow{7}{*}{RNN}    & Vanilla                 & 0.006           & 0.007             & 0.229             & 5.744    & 0.001    & 0.260 & 0.017    & 0.066    & 0.253 & 4.483    & 0.026    & 0.225  \\
                                                        &                         & Word-AT                 & 0.129           & 0.115             & 0.147             & 4.413    & 0.005    & 0.259 & 5.551    & 0.132    & 0.251 & 2.738    & 0.046    & 0.203  \\
                                                        &                         & Word-iAT                & 0.365           & 0.005             & 0.175             & 4.433    & 5.85E-04 & 0.258 & 2.178    & 0.091    & 0.246 & 2.804    & 0.091    & 0.203  \\
                                                        &                         & Attention-RP            & 0.099           & 0.073             & 0.142             & 6.001    & 2.87E-04 & 0.258 & 3.585    & 0.080    & 0.246 & 4.637    & 0.052    & 0.229  \\
                                                        &                         & Attention-AT            & 0.026           & 0.052             & 0.136             & 5.533    & 0.00E+00 & 0.259 & 2.493    & 0.372    & 0.252 & 0.008    & 0.049    & 0.236  \\
                                                        &                         & Attention-iAT           & 1.994           & 6.74E-04          & 0.215             & 4.788    & 0.00E+00 & 0.259 & 5.351    & 0.126    & 0.257 & 2.435    & 0.039    & 0.227  \\
                                                        &                         & SEAT(\textbf{Ours})     & 3.281           & 1.38E-05          & 0.134             & 6.016    & 0.00E+00 & 0.254 & 6.558    & 3.12E-04 & 0.133 & 4.713    & 9.20E-06 & 0.132  \\ 
\cmidrule{2-15}
                                                        & \multirow{7}{*}{BiLSTM} & Vanilla                 & 0.474           & 0.002             & 0.258             & 5.182    & 1.71E-04 & 0.258 & 4.916    & 0.112    & 0.260 & 2.966    & 0.088    & 0.224  \\
                                                        &                         & Word-AT                 & 1.756           & 0.006             & 0.259             & 4.939    & 0.009    & 0.260 & 2.743    & 0.115    & 0.259 & 2.666    & 0.137    & 0.228  \\
                                                        &                         & Word-iAT                & 1.765           & 0.025             & 0.259             & 5.082    & 2.62E-04 & 0.261 & 5.409    & 0.093    & 0.259 & 3.759    & 0.100    & 0.228  \\
                                                        &                         & Attention-RP            & 0.561           & 0.002             & 0.179             & 2.865    & 0.007    & 0.250 & 2.248    & 0.199    & 0.258 & 4.073    & 0.200    & 0.225  \\
                                                        &                         & Attention-AT            & 1.294           & 6.41E-04          & 0.252             & 2.129    & 0.004    & 0.259 & 3.220    & 0.178    & 0.259 & 4.925    & 0.216    & 0.236  \\
                                                        &                         & Attention-iAT           & 0.555           & 0.002             & 0.178             & 4.869    & 0.004    & 0.258 & 4.092    & 0.290    & 0.260 & 3.364    & 0.377    & 0.250  \\
                                                        &                         & SEAT(\textbf{Ours})     & 1.849           & 4.45E-04          & 0.169             & 5.435    & 4.37E-06 & 0.235 & 6.240    & 0.065    & 0.257 & 4.941    & 0.062    & 0.212  \\ 
\cmidrule{2-15}
                                                        & \multirow{7}{*}{BERT}   & Vanilla                 & 5.07E-04        & 0.008             & 0.021             & 0.003    & 0.310    & 0.015 & 3.20E-04 & 0.141    & 0.029 & 0.001    & 0.092    & 0.021  \\
                                                        &                         & Word-AT                 & 2.55E-05        & 0.012             & 0.017             & 7.64E-04 & 0.020    & 0.021 & 7.21E-04 & 0.023    & 0.026 & 7.75E-04 & 0.009    & 0.020  \\
                                                        &                         & Word-iAT                & 4.79E-04        & 0.013             & 0.024             & 9.51E-04 & 0.024    & 0.015 & 3.80E-04 & 0.012    & 0.028 & 6.15E-04 & 0.016    & 0.022  \\
                                                        &                         & Attention-RP            & 0.085           & 0.086             & 0.021             & 0.002    & 0.010    & 0.018 & 0.035    & 0.034    & 0.022 & 0.017    & 0.003    & 0.016  \\
                                                        &                         & Attention-AT            & 4.65E-05        & 0.003             & 0.017             & 7.31E-04 & 0.467    & 0.016 & 0.004    & 0.007    & 0.023 & 0.003    & 0.304    & 0.018  \\
                                                        &                         & Attention-iAT           & 6.23E-05        & 0.164             & 0.020             & 1.19E-04 & 9.07E-04 & 0.016 & 3.18E-04 & 0.151    & 0.021 & 0.003    & 0.025    & 0.017  \\
                                                        &                         & SEAT(\textbf{Ours})     & 0.160           & 0.002             & 0.017             & 0.497    & 0.00E+00 & 0.012 & 0.153    & 0.006    & 0.019 & 0.040    & 0.002    & 0.015  \\
\bottomrule
\end{tabular}
}
\caption{More results on the performance of different methods under different perturbation radii. Comprehensiveness, Sufficiency, and Sensitivity are reported to measure the model interpretability. From the table we can see that SEAT outperforms baseline models under all three metrics. It suggest that our method outperforms other baseline methods on model interpretability. \label{tab: more result other three metrics}}
\end{table*} 

==> SEAT_ Stable and Explainable Attention/tab/tab5.tex <==
\begin{table}
\centering
\resizebox{1.0\linewidth}{!}{\begin{tabular}{ccccccccc} 
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{7}{c}{\textbf{Method}}                                                                         \\ 
\cmidrule{3-9}
                         &                          & \textbf{Vanilla} & \textbf{W-AT} & \textbf{W-iAT} & \textbf{At-RP} & \textbf{At-AT} & \textbf{At-iAT} & \textbf{SEAT(Ours)}  \\ 
\midrule
\multirow{3}{*}{{Emotion}} & {JSD$\downarrow$}          & 0.628   & 0.004   & 0.456    & 0.039        & 0.082        & 0.126         & \textbf{1.72E-09}              \\
                         & {TVD$\downarrow$}          & 2.847   & 0.022   & 0.059    & 0.235        & 0.003        & 0.228         & {0.001}                 \\
                         & {F1$\uparrow$}             & {0.721}   & 0.694   & 0.658    & 0.657        & 0.707        & 0.684         & 0.714                 \\ 
\midrule
\multirow{3}{*}{{SST}}     & {JSD}                      & 0.315   & 0.175   & 0.213    & 0.089        & 0.006        & 0.147         & \textbf{1.55E-06}              \\
                         & {TVD}                      & 3.655   & 0.065   & 0.046    & 0.128        & 0.157        & 0.204         & \textbf{0.028}                 \\
                         & {F1}                       & 0.912   & 0.910   & 0.912    & 0.893        & 0.907        & \textbf{0.915}         & 0.907                 \\ 
\midrule
\multirow{3}{*}{{Hate}}    & JSD                      & 0.491   & 0.111   & 0.331    & 0.085        & 0.035        & 0.081         & \textbf{8.69E-06}              \\
                         & TVD                      & 2.004   & 0.058   & 0.044    & 0.278        & 0.230        & 0.271         & \textbf{0.037}                 \\
                         & F1                       & 0.493   & 0.546   & 0.501    & 0.554        & 0.510        & 0.512         & \textbf{0.555}                 \\ 
\midrule
\multirow{3}{*}{{RottenT}} & JSD                      & 0.585   & 0.473   & 0.488    & 0.078        & 0.049        & 0.136         & \textbf{1.10E-05}              \\
                         & TVD                      & 3.464   & 0.056   & 0.048    & 0.143        & 0.193        & 0.187         & \textbf{0.035}                 \\
                         & F1                       & 0.845   & 0.836   & \textbf{0.852}    & 0.817        & 0.818        & 0.831         & 0.847                 \\
\bottomrule
\end{tabular}}
\caption{
Results on the stability of BERT fine-tuned with different methods under word perturbation. JSD and TVD are reported to measure the stability while F1 measure the model accuracy on the clean data. The perturbation word size $K$ is set to 1 for each datasets. We denote "Attention" to "At" and "Word" to "W" for conveniently presented.}
\label{main_wordp}
\end{table}


==> SEAT_ Stable and Explainable Attention/tab/tab6.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccc} 
\toprule
\multirow{2}{*}{Perturb Word $N$} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Emotion}                                                             & \multicolumn{3}{c}{SST}  & \multicolumn{3}{c}{Hate} & \multicolumn{3}{c}{RottenT}  \\ 
\cmidrule(lr){3-5}\cmidrule(r){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
                                  &                         & JSD$\downarrow$ & TVD$\downarrow$ & F1$\uparrow$ & JSD      & TVD   & F1    & JSD      & TVD   & F1    & JSD      & TVD   & F1        \\ 
\midrule
\multirow{7}{*}{$N$=2}              & Vanilla                 & 0.628                        & 2.861                        & 0.721                     & 0.343    & 3.806 & 0.912 & 0.435    & 2.098 & 0.493 & 0.582    & 3.570 & 0.845     \\
                                  & Word-AT                 & 0.004                        & 0.022                        & 0.694                     & 0.175    & 0.065 & 0.910 & 0.111    & 0.058 & 0.546 & 0.473    & 0.056 & 0.836     \\
                                  & Word-iAT                & 0.456                        & 0.059                        & 0.658                     & 0.213    & 0.046 & 0.912 & 0.331    & 0.044 & 0.501 & 0.488    & 0.048 & 0.852     \\
                                  & Attention-RP            & 0.039                        & 0.235                        & 0.657                     & 0.089    & 0.128 & 0.893 & 0.085    & 0.278 & 0.554 & 0.078    & 0.143 & 0.817     \\
                                  & Attention-AT            & 0.082                        & 0.003                        & 0.707                     & 0.006    & 0.157 & 0.907 & 0.035    & 0.230 & 0.510 & 0.049    & 0.193 & 0.818     \\
                                  & Attention-iAT           & 0.126                        & 0.228                        & 0.684                     & 0.147    & 0.204 & 0.915 & 0.081    & 0.271 & 0.512 & 0.136    & 0.187 & 0.831     \\
                                 \rowcolor{grey!20} & SEAT (\textbf{Ours})    & 1.72E-09                     & 0.001                        & 0.716                     & 1.55E-06 & 0.028 & 0.906 & 8.69E-06 & 0.037 & 0.555 & 1.10E-05 & 0.035 & 0.849     \\ 
\midrule
\multirow{7}{*}{$N$=3}              & Vanilla                 & 0.618                        & 2.864                        & 0.721                     & 0.326    & 3.852 & 0.912 & 0.387    & 2.156 & 0.493 & 0.564    & 3.610 & 0.845     \\
                                  & Word-AT                 & 0.004                        & 0.022                        & 0.694                     & 0.175    & 0.065 & 0.910 & 0.111    & 0.058 & 0.546 & 0.473    & 0.056 & 0.836     \\
                                  & Word-iAT                & 0.456                        & 0.059                        & 0.658                     & 0.213    & 0.046 & 0.912 & 0.331    & 0.044 & 0.501 & 0.488    & 0.048 & 0.852     \\
                                  & Attention-RP            & 0.039                        & 0.235                        & 0.657                     & 0.089    & 0.128 & 0.893 & 0.085    & 0.278 & 0.554 & 0.078    & 0.143 & 0.817     \\
                                  & Attention-AT            & 0.082                        & 0.003                        & 0.707                     & 0.006    & 0.157 & 0.907 & 0.035    & 0.230 & 0.510 & 0.049    & 0.193 & 0.818     \\
                                  & Attention-iAT           & 0.126                        & 0.228                        & 0.684                     & 0.147    & 0.204 & 0.915 & 0.081    & 0.271 & 0.512 & 0.136    & 0.187 & 0.831     \\ 
                                 \rowcolor{grey!20} &  SEAT (\textbf{Ours})    & 1.72E-09                     & 0.001                        & 0.715                     & 1.55E-06 & 0.028 & 0.909 & 8.69E-06 & 0.037 & 0.555 & 1.10E-05 & 0.035 & 0.846     \\
\bottomrule
\end{tabular}}
\caption{More Results of evaluating stability of different methods under word perturbation.}
\label{tab_all_wordp}
\end{table*}


==> SEAT_ Stable and Explainable Attention/tab/tab7.tex <==
% \vspace{-10pt}
\begin{table*}
\renewcommand{\arraystretch}{0.8}
\centering
% \small
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccccccccccc} 
\toprule
 \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Emotion}}                                                             & \multicolumn{3}{c}{\textbf{SST}}  & \multicolumn{3}{c}{\textbf{Hate}} & \multicolumn{3}{c}{\textbf{RottenT}}  \\ 
\cmidrule(lr){2-4}\cmidrule(r){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
                                  &      \textbf{JSD$\downarrow$} & \textbf{TVD$\downarrow$} & \textbf{F1$\uparrow$} & \textbf{JSD} & \textbf{TVD}   & \textbf{F1}    & \textbf{JSD}      & \textbf{TVD}   & \textbf{F1}    & \textbf{JSD}      & \textbf{TVD}   & \textbf{F1}        \\ 
\midrule
  \textbf{Vanilla}           & 0.628                        & 2.847                        & \textbf{0.721}                     & 0.315    & 3.655 & 0.912 & 0.491    & 2.004 & 0.493 & 0.585    & 3.464 & 0.845     \\
                                   \textbf{Word-AT}                 & 0.004                        & 0.022                        & 0.694                     & 0.175    & 0.065 & 0.910 & 0.111    & 0.058 & 0.546 & 0.473    & 0.056 & 0.836     \\
                                   \textbf{Word-iAT}                & 0.456                        & 0.059                        & 0.658                     & 0.213    & 0.046 & 0.912 & 0.331    & 0.044 & 0.501 & 0.488    & 0.048 & \textbf{0.852}     \\
                                   \textbf{Attention-RP}            & 0.039                        & 0.235                        & 0.657                     & 0.089    & 0.128 & 0.893 & 0.085    & 0.278 & 0.554 & 0.078    & 0.143 & 0.817     \\
                                   \textbf{Attention-AT}            & 0.082                        & 0.003                        & 0.707                     & 0.006    & 0.157 & 0.907 & 0.035    & 0.230 & 0.510 & 0.049    & 0.193 & 0.818     \\
                                   \textbf{Attention-iAT}           & 0.126                        & 0.228                        & 0.684                     & 0.147    & 0.204 & \textbf{0.915} & 0.081    & 0.271 & 0.512 & 0.136    & 0.187 & 0.831     \\
                                 \rowcolor{grey!20}  \textbf{SEAT(Ours)}    & \textbf{1.72E-09}                     & \textbf{0.001}                        & 0.716                     & \textbf{1.55E-06} & \textbf{0.028} & 0.907 & \textbf{8.69E-06} & \textbf{0.037} & \textbf{0.555} & \textbf{1.10E-05} & \textbf{0.035} & 0.847     \\ 
\bottomrule
\end{tabular}}
\caption{Results on stability and utility of attention model trained with different methods under word perturbation. BERT is used as our architecture, and the perturbation word size is set as $N=1$. JSD, TVD, and F1 are reported.}
\label{tab_main_wordp}
\vspace{-12pt}
\end{table*}

==> figures/examples/embedding.tex <==

% code of example
\tikzset{
    %Define standard arrow tip
    >=stealth',
    %Define style for boxes
    punkt/.style={
          very thick,
          rectangle split,
          rectangle split parts=2,
          inner ysep=1.2mm,
          inner xsep=1.5mm,
          rounded corners,
          draw=black, thick,
          text width=9.3cm},
    punx/.style={
          rectangle,
          rounded corners,
          align=left,
          text width=0.55cm,
          text depth=0.01cm,
          draw=white},
  header/.style = {%
    inner ysep = +1.5em,
    append after command = {
      \pgfextra{\let\TikZlastnode\tikzlastnode}
      node [header node] (header-\TikZlastnode) at (\TikZlastnode.north) {#1}
      node [span = (\TikZlastnode)(header-\TikZlastnode)]
        at (fit bounding box) (h-\TikZlastnode) {}
    }
  },
}
\begin{tikzpicture}[scale=1.0]
\node[punkt](Vanilla){
\Textbox{0.1cm}{\textbf{Vanilla} \quad \textbf{JSD.$\downarrow$} = 0.024 \quad \textbf{TVD.$\downarrow$} = 2.321}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})
}\\
{\centering \small \textbf{Perturbed}: 
\colorword{pink!100}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!20}{black}{horrible}
($99.9\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Vanilla](Word-AT){
\Textbox{0.1cm}{\textbf{Word-AT} \quad \textbf{JSD.} = 0.078 \quad \textbf{TVD.} = 0.04}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% \colorword{pink}{black}{This} film is just plain {horrible}.
\colorword{pink!100}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!20}{black}{horrible}
($97.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\node[punkt, below=0cm of Word-AT](Att-AT){
\Textbox{0.1cm}{\textbf{Att-AT} \quad \textbf{JSD.} = 0.016 \quad \textbf{TVD.} = 0.237}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% {This} film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!60}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!70}{black}{horrible}
($67.9\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Att-AT](Ours){
\Textbox{0.1cm}{\textbf{Ours} \quad \textbf{JSD.} = 4.3e-7 \quad \textbf{TVD.} = 0.001}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!23}{black}{This} \colorword{pink!18}{black}{film} 
\colorword{pink!13}{black}{is} 
\colorword{pink!28}{black}{just}
\colorword{pink!48}{black}{plain} \colorword{pink!98}{black}{horrible}
($97.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\end{tikzpicture}

==> figures/examples/seed.tex <==

% code of example
\tikzset{
    %Define standard arrow tip
    >=stealth',
    %Define style for boxes
    punkt/.style={
          very thick,
          rectangle split,
          rectangle split parts=2,
          inner ysep=1.2mm,
          inner xsep=1.5mm,
          rounded corners,
          draw=black, thick,
          text width=9.3cm},
    punx/.style={
          rectangle,
          rounded corners,
          align=left,
          text width=0.55cm,
          text depth=0.01cm,
          draw=white},
  header/.style = {%
    inner ysep = +1.5em,
    append after command = {
      \pgfextra{\let\TikZlastnode\tikzlastnode}
      node [header node] (header-\TikZlastnode) at (\TikZlastnode.north) {#1}
      node [span = (\TikZlastnode)(header-\TikZlastnode)]
        at (fit bounding box) (h-\TikZlastnode) {}
    }
  },
}
\begin{tikzpicture}[scale=1.0]
\node[punkt](Vanilla){
\Textbox{0.1cm}{\textbf{Vanilla} \quad \textbf{JSD.$\downarrow$} = 0.008 \quad \textbf{TVD.$\downarrow$} = 0.172}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})
}\\
{\centering \small \textbf{Perturbed}: 
\colorword{pink!20}{black}{This} \colorword{pink!30}{black}{film} 
\colorword{pink!40}{black}{is} 
\colorword{pink!54}{black}{just}
\colorword{pink!20}{black}{plain} \colorword{pink!40}{black}{horrible}
($97.9\%\rightarrow$\textcolor{red}{\textcolor{blue}{Neg.}})}
};
\node[punkt, below=0cm of Vanilla](Word-AT){
\Textbox{0.1cm}{\textbf{Word-AT} \quad \textbf{JSD.} = 0.013 \quad \textbf{TVD.} = 0.080}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% \colorword{pink}{black}{This} film is just plain {horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!30}{black}{film} 
\colorword{pink!40}{black}{is} 
\colorword{pink!54}{black}{just}
\colorword{pink!20}{black}{plain} \colorword{pink!40}{black}{horrible}
($98.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\node[punkt, below=0cm of Word-AT](Att-AT){
\Textbox{0.1cm}{\textbf{Att-AT} \quad \textbf{JSD.} = 0.005 \quad \textbf{TVD.} = 0.189}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% {This} film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!40}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!50}{black}{horrible}
($95.9\%\rightarrow$\textcolor{red}{\textcolor{blue}{Neg.}})}
};
\node[punkt, below=0cm of Att-AT](Ours){
\Textbox{0.1cm}{\textbf{Ours} \quad \textbf{JSD.} = 6.5e-6 \quad \textbf{TVD.} = 0.013}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!30}{black}{This} \colorword{pink!25}{black}{film} 
\colorword{pink!13}{black}{is} 
\colorword{pink!28}{black}{just}
\colorword{pink!48}{black}{plain} \colorword{pink!98}{black}{horrible}
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\end{tikzpicture}

==> figures/examples/setup.tex <==

\colorlet{red1}{red}
\colorlet{red2}{red!50}
\colorlet{red3}{red!25}
\colorlet{blue1}{blue}
\colorlet{blue2}{blue!50}
\colorlet{blue3}{blue!25}
\makeatletter
\pgfdeclaregenericanchor{top base}{%
  \csname pgf@anchor@#1@north\endcsname
  \pgf@anchor@generic@top@base@main
}
\pgfdeclaregenericanchor{top base west}{%
  \csname pgf@anchor@#1@north west\endcsname
  \pgf@anchor@generic@top@base@main
}
\pgfdeclaregenericanchor{top base east}{%
  \csname pgf@anchor@#1@north east\endcsname
  \pgf@anchor@generic@top@base@main
}
\def\pgf@anchor@generic@top@base@main{%
  {%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y-\pgf@ya
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y-\pgf@ya
    \pgf@ya=0pt
    \pgfutil@loop
    \ifdim\pgf@y>\baselineskip
      \advance\pgf@y-\baselineskip
      \advance\pgf@ya\baselineskip
    \pgfutil@repeat
    \global\pgf@y=\pgf@ya
  }%
}
\makeatother
\newcommand\Textbox[2]{%
    \parbox[c][#1][c]{6.7cm}{#2}}


==> figures/examples/word.tex <==

% code of example
\tikzset{
    %Define standard arrow tip
    >=stealth',
    %Define style for boxes
    punkt/.style={
          very thick,
          rectangle split,
          rectangle split parts=2,
          inner ysep=1.2mm,
          inner xsep=1.5mm,
          rounded corners,
          draw=black, thick,
          text width=9.3cm},
    punx/.style={
          rectangle,
          rounded corners,
          align=left,
          text width=0.55cm,
          text depth=0.01cm,
          draw=white},
  header/.style = {%
    inner ysep = +1.5em,
    append after command = {
      \pgfextra{\let\TikZlastnode\tikzlastnode}
      node [header node] (header-\TikZlastnode) at (\TikZlastnode.north) {#1}
      node [span = (\TikZlastnode)(header-\TikZlastnode)]
        at (fit bounding box) (h-\TikZlastnode) {}
    }
  },
}
\begin{tikzpicture}[scale=1.0]
\node[punkt](Vanilla){
\Textbox{0.1cm}{\textbf{Vanilla} \quad \textbf{JSD.$\downarrow$} = 0.012 \quad \textbf{TVD.$\downarrow$} = 0.230}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\,
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})
}\\
{\centering \small \textbf{Perturbed}: 
\colorword{pink!30}{black}{This} \colorword{pink!20}{black}{\textbf{movie}} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!50}{black}{\textbf{terrible}}($59.2\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Vanilla](Word-AT){
\Textbox{0.1cm}{\textbf{Word-AT} \quad \textbf{JSD.} = 0.014 \quad \textbf{TVD.} = 0.080}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible}   
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% \colorword{pink}{black}{This} film is just plain {horrible}.
\colorword{pink!30}{black}{This} \colorword{pink!30}{black}{\textbf{movie}} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!40}{black}{plain} \colorword{pink!50}{black}{\textbf{terrible}}($99.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\node[punkt, below=0cm of Word-AT](Att-AT){
\Textbox{0.1cm}{\textbf{Att-AT} \quad \textbf{JSD.} = 0.004 \quad \textbf{TVD.} = 0.260}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!10}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!80}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% {This} film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{\textbf{movie}} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!30}{black}{plain} \colorword{pink!60}{black}{\textbf{terrible}}($56.8\%\rightarrow$\textcolor{red}{\textcolor{red}{Pos.}})}
};
\node[punkt, below=0cm of Att-AT](Ours){
\Textbox{0.1cm}{\textbf{Ours} \quad \textbf{JSD.} = 8.4e-8 \quad \textbf{TVD.} = 0.012}
\nodepart{second}
{\centering \small \textbf{Benign}:~~~\, 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!20}{black}{This} \colorword{pink!20}{black}{film} 
\colorword{pink!20}{black}{is} 
\colorword{pink!30}{black}{just}
\colorword{pink!50}{black}{plain} \colorword{pink!100}{black}{horrible} 
($99.9\%\rightarrow$\textcolor{blue}{Neg.})}\\
{\centering \small \textbf{Perturbed}: 
% This film is just plain \colorword{pink}{black}{horrible}.
\colorword{pink!23}{black}{This} \colorword{pink!18}{black}{\textbf{movie}} 
\colorword{pink!13}{black}{is} 
\colorword{pink!28}{black}{just}
\colorword{pink!48}{black}{plain} \colorword{pink!96}{black}{\textbf{terrible}}($98.9\%\rightarrow$\textcolor{blue}{Neg.})}
};
\end{tikzpicture}

==> figures/overview.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{figures/overview.pdf}
\caption{An illustration of an attention heatmap for a BiLSTM model with attention mechanisms and the model with REAL-attention. The proposed REAL-attention is more explainable for attention score and more stable for output distribution.}
\label{fig:overview}
\end{figure}

==> tab/tab5.tex <==
\begin{table}
\centering
\resizebox{1.0\linewidth}{!}{\begin{tabular}{ccccccccc} 
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{7}{c}{\textbf{Method}}                                                                         \\ 
\cmidrule{3-9}
                         &                          & \textbf{Vanilla} & \textbf{W-AT} & \textbf{W-iAT} & \textbf{At-RP} & \textbf{At-AT} & \textbf{At-iAT} & \textbf{SEAT(Ours)}  \\ 
\midrule
\multirow{3}{*}{{Emotion}} & {JSD$\downarrow$}          & 0.628   & 0.004   & 0.456    & 0.039        & 0.082        & 0.126         & \textbf{1.72E-09}              \\
                         & {TVD$\downarrow$}          & 2.847   & 0.022   & 0.059    & 0.235        & 0.003        & 0.228         & {0.001}                 \\
                         & {F1$\uparrow$}             & {0.721}   & 0.694   & 0.658    & 0.657        & 0.707        & 0.684         & 0.714                 \\ 
\midrule
\multirow{3}{*}{{SST}}     & {JSD}                      & 0.315   & 0.175   & 0.213    & 0.089        & 0.006        & 0.147         & \textbf{1.55E-06}              \\
                         & {TVD}                      & 3.655   & 0.065   & 0.046    & 0.128        & 0.157        & 0.204         & \textbf{0.028}                 \\
                         & {F1}                       & 0.912   & 0.910   & 0.912    & 0.893        & 0.907        & \textbf{0.915}         & 0.907                 \\ 
\midrule
\multirow{3}{*}{{Hate}}    & JSD                      & 0.491   & 0.111   & 0.331    & 0.085        & 0.035        & 0.081         & \textbf{8.69E-06}              \\
                         & TVD                      & 2.004   & 0.058   & 0.044    & 0.278        & 0.230        & 0.271         & \textbf{0.037}                 \\
                         & F1                       & 0.493   & 0.546   & 0.501    & 0.554        & 0.510        & 0.512         & \textbf{0.555}                 \\ 
\midrule
\multirow{3}{*}{{RottenT}} & JSD                      & 0.585   & 0.473   & 0.488    & 0.078        & 0.049        & 0.136         & \textbf{1.10E-05}              \\
                         & TVD                      & 3.464   & 0.056   & 0.048    & 0.143        & 0.193        & 0.187         & \textbf{0.035}                 \\
                         & F1                       & 0.845   & 0.836   & \textbf{0.852}    & 0.817        & 0.818        & 0.831         & 0.847                 \\
\bottomrule
\end{tabular}}
\caption{
Results on the stability of BERT fine-tuned with different methods under word perturbation. JSD and TVD are reported to measure the stability while F1 measure the model accuracy on the clean data. The perturbation word size $K$ is set to 1 for each datasets. We denote "Attention" to "At" and "Word" to "W" for conveniently presented.}
\label{main_wordp}
\end{table}

